Correctness Witnesses for Concurrent Programs: Bridging the Semantic Divide with Ghosts (Extended Version)

Static analyzers are typically complex tools and thus prone to contain bugs themselves. To increase the trust in the verdict of such tools, witnesses encode key reasoning steps underlying the verdict in an exchangeable format, enabling independent validation of the reasoning by other tools. For the correctness of concurrent programs, no agreed-upon witness format exists -- in no small part due to the divide between the semantics considered by analyzers, ranging from interleaving to thread-modular approaches, making it challenging to exchange information. We propose a format that leverages the well-known notion of ghosts to embed the claims a tool makes about a program into a modified program with ghosts, such that the validity of a witness can be decided by analyzing this program. Thus, the validity of witnesses with respect to the interleaving and the thread-modular semantics coincides. Further, thread-modular invariants computed by an abstract interpreter can naturally be expressed in the new format using ghost statements. We evaluate the approach by generating such ghost witnesses for a subset of concurrent programs from the SV-COMP benchmark suite, and pass them to a model checker. It can confirm 75% of these witnesses -- indicating that ghost witnesses can bridge the semantic divide between interleaving and thread-modular approaches.

==> content/table_existing_witnesses.tex <==
\begin{table}
    \caption{Existing witnesses in SV-COMP.}
    \label{tab:existing-witnesses}
    \centering
    \setlength{\tabcolsep}{2pt} % reduce acmart default
    \begin{tabular}{lcc}
        \toprule
        & \multicolumn{2}{c}{Witness type} \\
        \cmidrule(l){2-3} % trim looks weird without tabcolsep override
        Program type & Violation & Correctness \\
        \midrule
        Single-threaded & \citet{Beyer2015,Beyer_2022} & \citet{Beyer2016,Beyer_2022} \\
        Multithreaded & \citet{BeyerF20} & \emph{This work} \\
        \bottomrule
    \end{tabular}
\end{table}

==> figures/global-traces-ghost-program.tex <==

\begin{figure}[h!]
\ltDrawingDefs

% \scalebox{0.65}{
% 	\begin{tikzpicture}
% 	% Initial PP
% 	\node[programpointwide](tmpp0){};

% 	% Main thread
% 	\programon{tmpp0}{\create{$t_1$}}{tmpp1}
% 	% \programon{tmpp1}{\lock{l}}{tmpp2}
% 	% \programon{tmpp2}{\lock{$m_{u}$}}{tmpp3}
% 	% \programon[wide]{tmpp3}{\assert{\dots}}{tmpp4}
% 	% \programon[wide]{tmpp4}{\unlock{$m_{u}$}}{tmpp5}
% 	% \programon{tmpp5}{\unlock{l}}{tmpp6}

% 	% % Initial PPs
% 	\node[programpoint,below right=of tmpp1](t1pp0){};

% 	% % thread 1
% 	\programon{t1pp0}{\lock{l}}{t1pp1}
% 	\programon{t1pp1}{\lock{$m_{u}$}}{t1pp2}
% 	\programon[wide]{t1pp2}{used = 47}{t1pp3}
% 	% \programon{t1pp3}{\unlock{$m_{u}$}}{t1pp4}
% 	% \programon{t1pp4}{tmp++}{t1pp5}
% 	% \programon{t1pp5}{\lock{$m_{u}$}}{t1pp6}
% 	% \programon{t1pp6}{used = tmp}{t1pp7}

% 	\programondo{t1pp3}{}{t1pp14}
% 	% \programon{t1pp7}{\unlock{$m_{u}$}}{t1pp8}
% 	% \programon{t1pp8}{\lock{$m_{u}$}}{t1pp9}
% 	% \programon{t1pp9}{tmp = used}{t1pp10}
% 	% \programon{t1pp10}{\unlock{$m_{u}$}}{t1pp11}
% 	% \programon{t1pp11}{tmp--}{t1pp12}
% 	% \programon{t1pp12}{\lock{$m_{u}$}}{t1pp13}
% 	% \programon{t1pp13}{used = tmp}{t1pp14}

% 	\programon[wide]{t1pp14}{\unlock{$m_{u}$}}{t1pp15}
% 	\programon{t1pp15}{\unlock{l}}{t1pp16}
% 	\programon{t1pp16}{\code{printf(\dots)}}{t1pp17}

% 	% % create order
% 	\createo{tmpp0}{t1pp0}

% 	% % mutex orders
% 	% %% (m_used)
% 	\mutexo[above=0mm]{tmpp0}{t1pp2}{m_{u}}{out=-70,in=220}
% 	% \mutexo[above=0mm]{t1pp4}{t1pp6}{m_{u}}{out=320,in=220}
% 	% \mutexo[above=0mm]{t1pp8}{t1pp9}{m_{u}}{out=230,in=105}
% 	% \mutexo[above=0mm]{t1pp11}{t1pp13}{m_{u}}{out=230,in=105}
% 	% \mutexo[above=0mm]{t1pp15}{tmpp3}{m_{u}}{out=130,in=340}

% 	% %% (l)
% 	\mutexo{tmpp0}{t1pp1}{l}{out=-50,in=200}
% 	% \mutexo{t1pp16}{tmpp2}{l}{out=145,in=-40}

% \end{tikzpicture}}
\scalebox{0.65}{
	\begin{tikzpicture}
	% Initial PP
	\node[programpointwide](tmpp0){};

	% Main thread
	\programon{tmpp0}{\create{$t_1$}}{tmpp1}
	\programon{tmpp1}{\lock{l}}{tmpp2}
	\programon{tmpp2}{\lock{$m_{u}$}}{tmpp3}
	\programon[wide]{tmpp3}{\assert{\dots}}{tmpp4}
	\programon[wide]{tmpp4}{\unlock{$m_{u}$}}{tmpp5}
	\programon{tmpp5}{\unlock{l}}{tmpp6}

	% % Initial PPs
	\node[programpoint,below right=of tmpp1](t1pp0){};

	% % thread 1
	\programon{t1pp0}{\lock{l}}{t1pp1}
	\programon{t1pp1}{\lock{$m_{u}$}}{t1pp2}
	\programon[wide]{t1pp2}{used = 47}{t1pp3}
	% \programon{t1pp3}{\unlock{$m_{u}$}}{t1pp4}
	% \programon{t1pp4}{tmp++}{t1pp5}
	% \programon{t1pp5}{\lock{$m_{u}$}}{t1pp6}
	% \programon{t1pp6}{used = tmp}{t1pp7}

	\programondo{t1pp3}{}{t1pp14}
	% \programon{t1pp7}{\unlock{$m_{u}$}}{t1pp8}
	% \programon{t1pp8}{\lock{$m_{u}$}}{t1pp9}
	% \programon{t1pp9}{tmp = used}{t1pp10}
	% \programon{t1pp10}{\unlock{$m_{u}$}}{t1pp11}
	% \programon{t1pp11}{tmp--}{t1pp12}
	% \programon{t1pp12}{\lock{$m_{u}$}}{t1pp13}
	% \programon{t1pp13}{used = tmp}{t1pp14}

	\programon[wide]{t1pp14}{\unlock{$m_{u}$}}{t1pp15}
	\programon{t1pp15}{\unlock{l}}{t1pp16}
	% \programon[sink]{t1pp16}{printf(\dots)}{t1pp17}

	% % create order
	\createo{tmpp0}{t1pp0}

	% % mutex orders
	% %% (m_used)
	\mutexo[above=0mm]{tmpp0}{t1pp2}{m_{u}}{out=-70,in=220}
	% \mutexo[above=0mm]{t1pp4}{t1pp6}{m_{u}}{out=320,in=220}
	% \mutexo[above=0mm]{t1pp8}{t1pp9}{m_{u}}{out=230,in=105}
	% \mutexo[above=0mm]{t1pp11}{t1pp13}{m_{u}}{out=230,in=105}
	\mutexo[above=0mm]{t1pp15}{tmpp3}{m_{u}}{out=130,in=340}

	% %% (l)
	\mutexo{tmpp0}{t1pp1}{l}{out=-50,in=200}
	\mutexo{t1pp16}{tmpp2}{l}{out=145,in=-40}

\end{tikzpicture}}
\caption{A local trace of the program in \cref{listing:running-example}. Mutex $m_{used}$ is abbreviated with $m_u$. Here, the steps of $t_1$ some statements are omitted for clarity (indicated with the dotted arrow).}\label{fig:global-traces-ghost}
\end{figure}


==> figures/global-traces-program.tex <==

\begin{figure}[h!]
\ltDrawingDefs

\scalebox{0.65}{
\begin{tikzpicture}
	% Initial PP
	\node[programpointwide](tmpp0){};

	% Main thread
	\programon{tmpp0}{\create{$t_1$}}{tmpp1}
	\programon{tmpp1}{\lock{l}}{tmpp2}
	\programon{tmpp2}{\lock{$m_{u}$}}{tmpp3}
	\programon[wide]{tmpp3}{\assert{\dots}}{tmpp4}
	\programon[wide]{tmpp4}{\unlock{$m_{u}$}}{tmpp5}
	\programon{tmpp5}{\unlock{l}}{tmpp6}

	% % Initial PPs
	\node[programpoint,below right=of tmpp1](t1pp0){};

	% % thread 1
	\programon{t1pp0}{\lock{l}}{t1pp1}
	\programon{t1pp1}{\lock{$m_{u}$}}{t1pp2}
	\programon[wide]{t1pp2}{used = 47}{t1pp3}
	% \programon{t1pp3}{\unlock{$m_{u}$}}{t1pp4}
	% \programon{t1pp4}{tmp++}{t1pp5}
	% \programon{t1pp5}{\lock{$m_{u}$}}{t1pp6}
	% \programon{t1pp6}{used = tmp}{t1pp7}

	\programondo{t1pp3}{}{t1pp14}
	% \programon{t1pp7}{\unlock{$m_{u}$}}{t1pp8}
	% \programon{t1pp8}{\lock{$m_{u}$}}{t1pp9}
	% \programon{t1pp9}{tmp = used}{t1pp10}
	% \programon{t1pp10}{\unlock{$m_{u}$}}{t1pp11}
	% \programon{t1pp11}{tmp--}{t1pp12}
	% \programon{t1pp12}{\lock{$m_{u}$}}{t1pp13}
	% \programon{t1pp13}{used = tmp}{t1pp14}

	\programon[wide]{t1pp14}{\unlock{$m_{u}$}}{t1pp15}
	\programon{t1pp15}{\unlock{l}}{t1pp16}
	\programon{t1pp16}{\code{printf(\dots)}}{t1pp17}

	% % create order
	\createo{tmpp0}{t1pp0}

	% % mutex orders
	% %% (m_used)
	\mutexo[above=0mm]{tmpp0}{t1pp2}{m_{u}}{out=-70,in=220}
	% \mutexo[above=0mm]{t1pp4}{t1pp6}{m_{u}}{out=320,in=220}
	% \mutexo[above=0mm]{t1pp8}{t1pp9}{m_{u}}{out=230,in=105}
	% \mutexo[above=0mm]{t1pp11}{t1pp13}{m_{u}}{out=230,in=105}
	\mutexo[above=0mm]{t1pp15}{tmpp3}{m_{u}}{out=130,in=340}

	% %% (l)
	\mutexo{tmpp0}{t1pp1}{l}{out=-50,in=200}
	\mutexo{t1pp16}{tmpp2}{l}{out=145,in=-40}

\end{tikzpicture}}
\caption{Global trace of the program in \cref{listing:mutexes-example-program} without the ghost statements. Mutex $m_{used}$ is abbreviated with $m_u$. In the visualization the steps of $t_1$ belonging to the statements in lines 25-36 are omitted for clarity (indicated with the dotted arrow).}\label{fig:global-trace}
\end{figure}


==> figures/proof_overview_fig.tex <==
\begin{figure}
  \usetikzlibrary{positioning}

  \centering
  \begin{tikzpicture}
    \node (1)               {$\InterleavingExecutions_{\LanguageWithMg}$};
    \node (2) [below=of 1]  {$\LocalTraces$};
    \node (3) [right=of 1]  {$\InterleavingExecutions_{\LanguageWithoutMg}$};
    \node (4) [right=of 3]  {$\InterleavingExecutions_{Ghost^E}$};
    \node (5) [right=of 4]  {$\InterleavingExecutions_{\LanguageWithMg + Ghost^M}$};
    \node (6) [below=of 5]  {$\LocalTraces_{Ghost^M}$};

    \begin{scope}[nodes={font=\tiny, align=left, text width=2cm}]
      \draw (1) edge[<->] node[above]{\cref{interleaving-local-trace-equiv}} (2);
      \path (1) edge[<->] node[midway, above]{\cref{relation-interl-w/o-mg}} (3);
      \path (3) edge[<->] node[above]{There is a bijection (\cref{equiv-I-IG})} (4);
      \path ([yshift=1mm] 4.east) edge[->] node[above, yshift=1mm]{Transformation exists (\cref{inclusion-ghost-into-atomicity-mutexes}), but introduces deadlocks involving $\MutexesForGlobals$ mutexes} ([yshift=1mm] 5.west);
      \draw ([yshift=-1mm] 5.west) edge[->] node[below, yshift=-1mm]{Equivalent interleaving is constructed by projecting away mutexes in $\MutexesForGlobals$ and operations on these (\cref{lemma:interleaving-ghost-mutexes-to-atomicity}).} ([yshift=-1mm] 4.east);
      \path (6) edge[<->] node[above]{\cref{interleaving-local-trace-equiv}}  (5);
    \end{scope}

  \end{tikzpicture}
	\caption{Overview over proof. $Ghost^E$ indicates that ghosts are added via atomic ghost edges whereas $Ghost^M$ indicates that atomicity is encoded with mutexes.}
\end{figure}


==> tables/structure-ghost-updates.tex <==
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{3.5pt}
\setlength{\multilen}{6.5cm}
\begin{tabular}{lll}
  \toprule
  Key & Value & Description \\
  \midrule
  \ttbox{ghost\_updates}   & array                 & the list of \ttbox{ghost\_update} items; see below \\
  %
  \separator{content of \ttbox{ghost\_update}} \\
  \ttbox{location}         & mapping               & the location of the ghost update as structured in~\cite{Ayaziova2024} \\
  \ttbox{updates}          & array                 & the list of \ttbox{update} items; see below \\
  %
  \separator{content of \ttbox{update}} \\
  \ttbox{variable}         & scalar                & the name of the ghost variable \\
  \ttbox{value}            & scalar                & the value assigned to the ghost variable \\
  \ttbox{format}           & \ttbox{c\_expression} & the format is always \ttbox{c\_expression} \\
  \bottomrule
\end{tabular}


==> tables/structure-ghost-variables.tex <==
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{3.5pt}
\setlength{\multilen}{6.5cm}
\begin{tabular}{lll}
  \toprule
  Key & Value & Description \\
  \midrule
  \ttbox{ghost\_variables} & array                 & the list of \ttbox{ghost\_variable} items; see below \\
  %
  \separator{content of \ttbox{ghost\_variable}} \\
  \ttbox{name}             & scalar                & the name of the ghost variable \\
  \ttbox{type}             & scalar                & the type of the ghost variable \\
  \ttbox{scope}            & \ttbox{global}        & the scope of the ghost variable is always \ttbox{global} \\
  \ttbox{initial}          & mapping               & the initial value of the ghost variable; see below \\
  %
  \separator{content of \ttbox{initial}} \\
  \ttbox{value}            & scalar                & the initial value of the ghost variable \\
  \ttbox{format}           & \ttbox{c\_expression} & the format is always \ttbox{c\_expression} \\
  \bottomrule
\end{tabular}

